HEX: Human-in-the-loop Explainability via Deep Reinforcement Learning

The use of machine learning (ML) models in decision-making contexts, particularly those used in high-stakes decision-making, are fraught with issue and peril since a person - not a machine - must ultimately be held accountable for the consequences of the decisions made using such systems. Machine learning explainability (MLX) promises to provide decision-makers with prediction-specific rationale, assuring them that the model-elicited predictions are made for the right reasons and are thus reliable. Few works explicitly consider this key human-in-the-loop (HITL) component, however. In this work we propose HEX, a human-in-the-loop deep reinforcement learning approach to MLX. HEX incorporates 0-distrust projection to synthesize decider specific explanation-providing policies from any arbitrary classification model. HEX is also constructed to operate in limited or reduced training data scenarios, such as those employing federated learning. Our formulation explicitly considers the decision boundary of the ML model in question, rather than the underlying training data, which is a shortcoming of many model-agnostic MLX methods. Our proposed methods thus synthesize HITL MLX policies that explicitly capture the decision boundary of the model in question for use in limited data scenarios.

==> coverletter.tex <==
\input{jmlr_coverletter_preamble.tex}

\begin{document}
\hfill{\today}

Journal of Machine Learning Research

\bigskip

Dear Editors:

We are writing to submit our manuscript ``\red{HEX: Human-in-the-loop Explainability via Deep Reinforcement Learning}'' to the \emph{Journal of Machine Learning Research}.

Our manuscript studies \red{machine learning explainability (MLX)}. We formulate the MLX problem as a Markov decision process (MDP) and adopt a \red{deep reinforcement learning (DRL)} approach to synthesize machine learning (ML) model-agnostic MLX policies. By learning MLX policies in this manner, we overcome the computational issues of competing approaches that learn local, instance-specific surrogate models (i.e.,~learn one model for each instance in need of explanation).

Our proposed formulation centers on the search for an \red{explanatory point}, the point on the decision boundary of the ML model in question nearest the instance being explained. The explanatory point produces explanations that are specific to the ML model, rather than the training data, a common short-coming of model-agnostic MLX methods (i.e.,~many model-agnostic MLX methods explain the underlying training data, rather than the ML model in question).

Our problem setting specifically considers a \red{human-in-the-loop (HITL)} decider, which is an under-studied, yet central aspect to MLX -- i.e.,~MLX is only needed because of a HITL, otherwise explanations would not be needed. Our formulation considers the preferred features of the HITL decider by defining the domain of these features as the feasible explanation region and projecting onto this domain when learning MLX policies. Our proposed method therefore learns decider-specific (i.e.,~human-specific) MLX policies.

Finally, our problem setting and method considers a limited data scenario, where the data available to produce explanations (and learn MLX policies) is a subset of, or different from, that used to train the ML model in question. We motivate and adopt this scenario by considering the high stakes decision-making use-cases of MLX, such as health care, and recent ML advances employed in these contexts, such as \red{federated learning}. Our proposed DRL approach explores the probability space during training, thus mitigating this limited data concern. We also adopt a procedure to overcome any persistent class imbalance.


We suggest the following action editors and referees for our submission.

Action Editors:
\begin{itemize}
    \item \red{Manuel Gomez-Rodriguez, Max Planck Institute for Software Systems (manuel@mpi-sws.org)}
    \item \red{Adrian Weller, University of Cambridge & The Alan Turing Institute (adrian.weller@eng.cam.ac.uk)}
    \item \red{Pradeep Ravikumar, Carnegie Mellon University (pradeepr@cs.cmu.edu)}
    \item \red{Florence d'Alché-Buc, Telecom Paris, Institut Polytechnique de Paris (florence.dalche@telecom-paris.fr)}
    \item \red{David Jensen, University of Massachusetts Amherst (jensen@cs.umass.edu)}
\end{itemize}

Reviewers:
\begin{itemize}
    \item \red{Przemyslaw Biecek, Warsaw University of Technology (przemyslaw.biecek@gmail.com)}
    \item \red{Maximilian Alber, Technische Universität Berlin (maximilian.alber@tu-berlin.com)}
    \item \red{Pieter-Jan Kindermans, Google Brain (pikinder@google.com)}
    \item \red{Xiaoqian Wang, Purdue University (joywang@purdue.edu)}
\end{itemize}

Our submission has the following keywords: \red{explainability}, \red{human-in-the-loop}, \red{deep reinforcement learning}, \red{federated learning}, \red{interpretability}.

As the corresponding author, I confirm that none of the co-authors listed below have a conflict of interest with the action editors and referees I suggest above. Further, I confirm that all co-authors below consent to my submission of this manuscript to the \emph{Journal of Machine Learning Research}.

\bigskip

Sincerely,

\medskip

\red{Michael T.~Lash (University of Kansas)}

\end{document}


















